Improving Minimum Bayes Risk Decoding with Multi-Prompt

While instruction fine-tuned LLMs are effective text generators, sensitivity to prompt construction makes performance unstable and sub-optimal in practice. Relying on a single "best" prompt cannot capture all differing approaches to a generation problem. Using this observation, we propose multi-prompt decoding, where many candidate generations are decoded from a prompt bank at inference-time. To ensemble candidates, we use Minimum Bayes Risk (MBR) decoding, which selects a final output using a trained value metric. We show multi-prompt improves MBR across a comprehensive set of conditional generation tasks, and show this is a result of estimating a more diverse and higher quality candidate space than that of a single prompt. Further experiments confirm multi-prompt improves generation across tasks, models and metrics.

==> fig/diversity_per_task.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=0.4\textwidth]{img/diversity_per_task.pdf}
\setlength{\abovecaptionskip}{5pt}
\setlength{\belowcaptionskip}{-10pt}
\captionof{figure}{Candidate set diversity and \textsc{BARTScore} on tasks from \citet{suzgun-etal-2023-follow}. Fitting value metrics becomes easier to fit for tasks where candidate diversity is drawn out by multi-prompt.}
\label{fig:diversity_per_task}
\end{figure}

==> tab/multi_model_large.tex <==
\begin{table*}[t!]
\centering
\small
% \fontsize{8}{9.5}\selectfont

\begin{tabular}{L{75pt}C{55pt}C{55pt}C{55pt}C{55pt}}
\toprule
 & Single Prompt & Multi\nobreakdash-prompt & Cand. \textsc{Bleu} (MP on SP) & Cand. \textsc{Bleu} (SP on MP) \\
\midrule
\multicolumn{5}{l}{\textit{Code Generation} ($|\mathcal{H}|\!=\!20$) -- \textsc{HumanEval} (pass@1)} \\
\hdashrule
StarCoder 2 15B     & 44.51 & 49.39 (\plus{4.88}) & 49.69 & 50.13 \\
CodeLlama 7B        & 37.80 & 40.85 (\plus{3.05}) & 62.05 & 63.32 \\
CodeLlama 13B       & 43.29 & 48.17 (\plus{4.88}) & 59.49 & 60.76 \\
CodeLlama 34B       & 45.73 & 52.44 (\plus{6.71}) & 61.59 & 62.92 \\
CodeLlama 70B       & 61.59 & 68.90 (\plus{7.31}) & 63.15 & 65.12 \\
GPT-3.5             & 68.29 & 73.78 (\plus{5.49}) & 83.07 & 89.86 \\
GPT-4               & 81.71 & 82.93 (\plus{1.22}) & 81.72 & 89.82 \\
\midrule
\multicolumn{5}{l}{\textit{Text Simplification} ($|\mathcal{H}|\!=\!100$) -- \textsc{SimpEval} (LENS)} \\
\hdashrule
Ctrl T5 3B          & 72.6 & -- & -- & -- \\
Ctrl T5 11B         & 74.4 & -- & -- & -- \\
Llama 2 7B Chat     & 75.71 & 80.38 (\plus{4.67}) & 80.71 & 74.68 \\
Llama 2 13B Chat    & 78.19 & 80.27 (\plus{2.08}) & 79.30 & 77.65 \\
Llama 2 70B Chat    & 82.21 & 83.28 (\plus{1.07}) & 74.11 & 70.65 \\
GPT-3.5             & 76.87 & 81.25 (\plus{4.38}) & 94.18 & 85.56 \\
GPT-4               & 76.47 & 81.56 (\plus{5.09}) & 96.74 & 81.05 \\
\midrule
\multicolumn{5}{l}{\textit{Translation} ($|\mathcal{H}|\!=\!100$) -- WMT '22 \textsc{En-Cs} (COMET)} \\
\hdashrule
WMT '22 Winners     & 91.9 & -- & -- & -- \\
MS Translate API    & 90.6 & -- & -- & -- \\
ALMA 7B R           & 89.17 & 89.94 (\plus{0.77}) & 87.22 & 81.20 \\
ALMA 13B R          & 89.41 & 90.45 (\plus{1.04}) & 89.75 & 84.74 \\
GPT-3.5             & 91.27 & 91.35 (\plus{0.08}) & 99.26 & 95.47 \\
GPT-4               & 92.24 & 92.47 (\plus{0.23}) & 90.21 & 90.85 \\
% TowerInstruct 7B    & 86.69 & 88.58 \\
% TowerInstruct 13B   & 88.92 & 90.00 \\
% Aya 101             & 90.27 & 90.68 \\
\bottomrule
\end{tabular}
\setlength{\belowcaptionskip}{-10pt}
\caption{Metric scores for state-of-the-art systems compared to LLMs with multi-prompt using $|\mathcal{H}|$ candidates. Translation and simplification baselines are as reported in \citet{hendy2023good} and \citet{maddela-etal-2023-lens}.}
\label{table:multi_model}
\end{table*}

==> tab/multi_model_old.tex <==
\begin{table}[t!]
\centering
\small
\begin{tabular}{L{75pt}C{55pt}C{55pt}}
\toprule
 & Single Prompt & Multi\nobreakdash-prompt \\
\midrule
\multicolumn{3}{l}{\textit{Code Generation} ($|\mathcal{H}|\!=\!20$) -- \textsc{HumanEval} (pass@1)} \\
StarCoder 2 15B     & 44.51 & 49.39 (\plus{4.88}) \\
CodeLlama 7B        & 37.80 & 40.85 (\plus{3.05}) \\
CodeLlama 13B       & 43.29 & 48.17 (\plus{4.88}) \\
CodeLlama 34B       & 45.73 & 52.44 (\plus{6.71}) \\
CodeLlama 70B       & 61.59 & 68.90 (\plus{7.31}) \\
GPT-3.5             & 68.29 & 73.78 (\plus{5.49}) \\
GPT-4               & 81.71 & 82.93 (\plus{1.22}) \\
\midrule
\multicolumn{3}{l}{\textit{Text Simplification} ($|\mathcal{H}|\!=\!100$) -- \textsc{SimpEval} (LENS)} \\
Ctrl T5 3B          & 72.6 & -- \\
Ctrl T5 11B         & 74.4 & -- \\
Llama 2 7B Chat     & 75.71 & 80.38 (\plus{4.67}) \\
Llama 2 13B Chat    & 78.19 & 80.27 (\plus{2.08}) \\
Llama 2 70B Chat    & 82.21 & 83.28 (\plus{1.07}) \\
GPT-3.5             & 76.87 & 81.25 (\plus{4.38}) \\
GPT-4               & 76.47 & 81.56 (\plus{5.09}) \\
\midrule
\multicolumn{3}{l}{\textit{Translation} ($|\mathcal{H}|\!=\!100$) -- WMT '22 \textsc{En-Cs} (COMET)} \\
WMT '22 Winners     & 91.9 & -- \\
MS Translate API    & 90.6 & -- \\
ALMA 7B R           & 89.17 & 89.94 (\plus{0.77}) \\
ALMA 13B R          & 89.41 & 90.45 (\plus{1.04}) \\
GPT-3.5             & 91.27 & 91.35 (\plus{0.08}) \\
GPT-4               & 92.24 & 92.47 (\plus{0.23}) \\
\bottomrule
\end{tabular}
\setlength{\belowcaptionskip}{-10pt}
\caption{Metric scores for state-of-the-art systems compared to LLMs with multi-prompt using $|\mathcal{H}|$ candidates. Translation and simplification baselines are as reported in \citet{hendy2023good} and \citet{maddela-etal-2023-lens}.}
\label{table:multi_model}
\end{table}
